High-Throughput Synchronous Deep RL

Deep reinforcement learning (RL) is computationally demanding and requires processing of many data points. Synchronous methods enjoy training stability while having lower data throughput. In contrast, asynchronous methods achieve high throughput but suffer from stability issues and lower sample efficiency due to `stale policies.' To combine the advantages of both methods we propose High-Throughput Synchronous Deep Reinforcement Learning (HTS-RL). In HTS-RL, we perform learning and rollouts concurrently, devise a system design which avoids `stale policies' and ensure that actors interact with environment replicas in an asynchronous manner while maintaining full determinism. We evaluate our approach on Atari games and the Google Research Football environment. Compared to synchronous baselines, HTS-RL is 2-6$\times$ faster. Compared to state-of-the-art asynchronous methods, HTS-RL has competitive throughput and consistently achieves higher average episode rewards.

==> atari_results.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{4pt}
{\small
\begin{tabular}{l|rrr}
\specialrule{.15em}{.05em}{.05em}
         Method &  IMPALA  &      A2C &  Ours (A2C)\\
\hline
\hline

 Space. &   542 $\pm$ 157&    596 $\pm$ 69 &      \bf{731} $\pm$ 80  \\
       Seaquest&   458 $\pm$ 2  &   \bf{1833 $\pm$ 6} &     1831 $\pm$ 7 \\
          Qbert &  4116 $\pm$ 610 &   12479 $\pm$ 1965 &    \bf{13682 $\pm$ 1873}  \\
       Breakout&   201 $\pm$ 133 &    362 $\pm$ 29 &      \bf{413 $\pm$ 37}  \\
     Beam Rider&  1997 $\pm$ 306 &   4392 $\pm$ 134 &     \bf{6995} $\pm$ 420  \\
      BankHeist&  339 $\pm$ 10 &   775 $\pm$ 166 &     \bf{942 $\pm$ 100}   \\
       MsPacman&   807 $\pm$ 170 &   1236 $\pm$ 292 &     \bf{1675 $\pm$ 459}  \\
      Jamesbond&    82 $\pm$ 10 &    438 $\pm$ 59 &      \bf{474 $\pm$ 88}  \\
   KFMaster&  9516 $\pm$ 3311 &  \bf{30752 $\pm$ 6641} &    30020 $\pm$ 3559  \\
    Star Gunner&  5350 $\pm$ 918 &  41414 $\pm$ 3826 &    \bf{52666 $\pm$ 5182}  \\
          Krull &  2546 $\pm$ 551 &   7560 $\pm$ 892 &     \bf{7737 $\pm$ 609}  \\
      Frostbite&    73 $\pm$ 2 &    272 $\pm$ 14&      \bf{315 $\pm$ 12}  \\
\specialrule{.15em}{.05em}{.05em}
\end{tabular}
\caption{{Atari experiment in \emph{final time metrics}: }Average evaluation rewards achieved given limited training time. The time limit for each experiment is set to the time when IMPALA finishes training for 20M  steps. Space.: Space invaders, KFMaster: KungFu Master.
}
\label{tab:atari_results}
}
\end{table}

==> atari_results_v2.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{llllllllllll}
\specialrule{.15em}{.05em}{.05em}
 Space Invaders &  Seaquest &    Qbert &  Breakout &  Beam Rider &  BankHeist &  MsPacman &  Jamesbond &  KungFuMaster &  Star Gunner &   Krull &  Frostbite \\
 \hline
 \hline
          595.2 &    1833.3 &   4168.7 &     362.5 &      4606.6 &     1993.7 &    1406.2 &        438 &         30752 &        41414 &  7461.7 &        272 \\
          765.1 &    1831.2 &  10076.2 &     413.4 &     5903.15 &     2401.3 &    1757.2 &        474 &         24016 &        52666 &  7497.5 &      315.8 \\
          709.9 &       458 &     4116 &     201.6 &        1997 &     1695.2 &     807.6 &         82 &          9516 &         5350 &    2546 &       73.2 \\
\specialrule{.15em}{.05em}{.05em}
\end{tabular}



\caption{\todo{Write something.}}
\label{tab:atari_results}
\end{table*}

==> exp_var_actor.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.22\textwidth, trim={0.6cm 0.5cm 0.2cm 0.},clip]{fig/stv_ours_ppo.pdf}
\includegraphics[height=2.85cm, width=0.25\textwidth, trim={0.6cm 0.5cm 0.2cm 0.8cm},clip]{fig/sps_noe.pdf}
\vspace{-1em}
\caption{\textbf{Left:} RTH-RL \as{what is `RTH-RL'?} speed up versus environment step time variance. RTS: `Run to score', 3v1: `3 versus 1 with keeper', CA hard: `Conner attack hard'.  \textbf{Right:} Step per second (SPS) versus  number of environments in GFootball `counterattack hard' scenario.
\as{better combine this with Fig.~3 into a single row of five plots across two columns of text? this will safe some space}
}
\label{fig:sps}

\end{figure}

==> football_results.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{4pt}
{\small
\begin{tabular}{l|rrr}
\specialrule{.15em}{.05em}{.05em}
         Method & IMPALA  &      PPO &  \makecell{Ours (PPO)}\\
\hline
\hline
{Empty goal close} & 1.7/2.6&    5.4/15.5 &      \bf{1.0/2.0}  \\
                         
{Empty goal}  & 8.4/11.7&    12.8/19.2 &      \bf{2.0/3.9}  \\
                           
{Run to score}  & 27.0/34.6&    16.2/32.5 &      \bf{6.3/11.4}  \\             
                                       
{RSK}  & 52.3/-&    51.2/68.2 &      \bf{11.5/18.8} \\

{PSK}  & -/-&    70.0/- &      {\bf{38.8}}/-  \\

{RPSK} & 22.3/\bf{25.4}&    45.2/90.8 &      {\bf{13.5}}/27.1  \\
     
{3 vs 1 w/ keeper}  & -/-&    67.4/144.2 &      \bf{15.9/25.6}\\
    
{Corner}  & -/-&    -/- &      -/- \\
                   
{Counterattack easy} & -/-&    223.2/- &      {\bf{91.3}}/- \\
                        
{Counterattack hard}  & -/-&    383.4/- &      \bf{61.8/-}  \\
{11 vs 11 w/ lazy Opp.}  &58.2/-&    95.8/260.9 &      \bf{14.4/72.1} \\
\specialrule{.15em}{.05em}{.05em}
\end{tabular}
\caption{GFootball experiments in \emph{required time metrics:} required time (minutes) to achieve goal scores (time required to achieve score 0.4 / time required to achieve score 0.8).  `-' represents the method did not achieve the desired score after 5M environment step training. RSK: run to score w/ keeper, PSK: pass, shoot, w/ keeper, RPSK: run, pass, shoot, w/ keeper.
}
\label{tab:football_results}
}
\end{table}
